SA-ConvONet: Sign-Agnostic Optimization of Convolutional Occupancy Networks

Surface reconstruction from point clouds is a fundamental problem in the computer vision and graphics community. Recent state-of-the-arts solve this problem by individually optimizing each local implicit field during inference. Without considering the geometric relationships between local fields, they typically require accurate normals to avoid the sign conflict problem in overlapped regions of local fields, which severely limits their applicability to raw scans where surface normals could be unavailable. Although SAL breaks this limitation via sign-agnostic learning, further works still need to explore how to extend this technique for local shape modeling. To this end, we propose to learn implicit surface reconstruction by sign-agnostic optimization of convolutional occupancy networks, to simultaneously achieve advanced scalability to large-scale scenes, generality to novel shapes, and applicability to raw scans in a unified framework. Concretely, we achieve this goal by a simple yet effective design, which further optimizes the pre-trained occupancy prediction networks with an unsigned cross-entropy loss during inference. The learning of occupancy fields is conditioned on convolutional features from an hourglass network architecture. Extensive experimental comparisons with previous state-of-the-arts on both object-level and scene-level datasets demonstrate the superior accuracy of our approach for surface reconstruction from un-orientated point clouds. The code is available at https://github.com/tangjiapeng/SA-ConvONet.

==> ICCV2021 Sign Agnostic ConvONet/ablation.tex <==
%\subsection{Ablation Studies}
%\noindent \textbf{Effective of Network Pretraining for Optimizing ConvONet}
%\noindent \textbf{Curvature-Adaptive point sampling for preserving fine details}

% \subsection{Robustness Evaluation} 
%     \noindent \textbf{point sets of varying noise levels.}
%     \noindent \textbf{point sets of varying sizes.}

==> ICCV2021 Sign Agnostic ConvONet/abstract.tex <==


%%%%%%%%% ABSTRACT
\begin{abstract}
    % Previous version submiited in the abstract ddl.
    % Surface reconstruction from point clouds is a fundamental problem in the computer vision and graphics community. Recent state-of-art methods~\cite{jiang2020local, chabra2020deep, tretschk2020patchnets} try to solve this problem by individually optimizing learned local implicit fields at the test time. Without considering the geometric relationships between local fields, they heavily rely on accurate normals to avoid the sign conflict problem in the overlapped regions of local fields, which seriously limits their applicability to raw scans where orientations of points could be unavailable or noisy. To this end, we propose to optimize the local implicit fields that are learned from convolutional features of U-Net from unsigned inputs. Our key insight is that geometric consistency between local fields are enforced implicitly by learning their encoding in a hourglass convolutional manner, which guarantees the assembled local field as a globally consistent one. 
    % Based on the learned geometric prior that avoids the sign flipping problem of local fields,
    % we design a self-supervised objective to maximize the consistency between learned local implicit fields and input observation without the use of normals during inference.
    % Extensive comparisons against previous state-of-the-arts on both object-level and scene-level datasets demonstrate the superior accuracy of our approach for surface reconstruction from un-orientated point clouds.
    
    Surface reconstruction from point clouds is a fundamental problem in the computer vision and graphics community. Recent state-of-the-arts solve this problem by individually optimizing each local implicit field during inference. Without considering the geometric relationships between local fields, they typically require accurate normals to avoid the sign conflict problem in overlapped regions of local fields, which severely limits their applicability to raw scans where surface normals could be unavailable. 
    Although SAL breaks this limitation via sign-agnostic learning, further works still need to explore how to extend this technique for local shape modeling.
    To this end, we propose to learn implicit surface reconstruction by sign-agnostic optimization of convolutional occupancy networks, to simultaneously achieve advanced scalability to large-scale scenes, generality to novel shapes, and applicability to raw scans in a unified framework. Concretely, we achieve this goal by a simple yet effective design, which further optimizes the pre-trained occupancy prediction networks with an unsigned cross-entropy loss during inference. The learning of occupancy fields is conditioned on convolutional features from an hourglass network architecture.
    Extensive experimental comparisons with previous state-of-the-arts on both object-level and scene-level datasets demonstrate the superior accuracy of our approach for surface reconstruction from un-orientated point clouds. The code is available at {\url{ https://github.com/tangjiapeng/SA-ConvONet}}.
   
   
   %Surface reconstruction from point clouds is a fundamental problem in the computer vision and graphics community. Recent state-of-the-arts solve this problem by individually optimizing each local implicit field during inference. Without considering the geometric relationships between local fields, they typically require accurate normals to avoid the sign conflict problem in overlapping regions of local fields, which severely limits their applicability to raw scans where surface normals could be unavailable. Although SAL breaks this limitation via sign-agnostic learning, it is still unexplored that how to extend this pipeline to local shape modeling. To this end, we propose to learn implicit surface reconstruction by sign-agnostic optimization of convolutional occupancy networks, to simultaneously achieve advanced scalability, generality, and applicability in a unified framework. In the paper, we also show this goal can be effectively achieved by a simple yet effective design, which optimizes the occupancy fields that are conditioned on convolutional features from an hourglass network architecture with an unsigned binary cross-entropy loss. Extensive experimental comparison with previous state-of-the-arts on both object-level and scene-level datasets demonstrate the superior accuracy of our approach for surface reconstruction from un-orientated point clouds.
\end{abstract}

==> ICCV2021 Sign Agnostic ConvONet/approach.tex <==
\section{Approach}
\label{SecApp}

\subsection{Overview}
\label{SubSecOver}
    Given a set of observed points $\mathcal{P} = \{\mathbf{p}_i \in \mathbb{R}^3 \}_{i=1}^n$, the goal of our method is to reconstruct a surface $\mathcal{S}$ that is as similar as possible to the underlying surface $\hat{\mathcal{S}}$. We choose to approximate the signed implicit field representation $\hat{\mathbf{O}}$ of $\hat{\mathcal{S}}$ by predicting a neural implicit field $\mathcal{O}$ due to its advantage of reconstructing surfaces with infinite resolution and unrestricted topology.
    Our goal is to simultaneously achieve advancements in all three respects, \tang{\ie scalability to large-scale scenes, generality to novel shapes, and applicability to raw scans}. 
    Towards this goal,  we propose a simple yet effective solution of learning implicit surface reconstructions by sign-agnostic optimization of convolutional occupancy networks.  
    % Firstly, our method performs local geometry modeling \dan{to} enable the scalability \dan{for application in} large-scale scenes. Secondly, our method effectively breaks the barrier of pre-trained priors by further optimizing network parameters for the given input during inference. This can maximize the generality to novel shapes, \dan{and improve the generation details of complicated surfaces}.
    % Lastly, our method \dan{achieves} the sign-agnostic implicit surface optimization directly from un-oriented point clouds, which \dan{clearly enhances} the practical applicability to \dan{real-world} scans where surface normals are \dan{quite} possibly unavailable.
    
    The overall pipeline \dan{of the proposed approach} is shown in Figure~\ref{fig:pipeline}.
   %\dan{It} is built on the convolutional occupancy networks~\cite{peng2020convolutional} that predicts an occupancy field $\mathbf{O}$ based on convolutional features $\mathbf{V}$ extracted from the input point cloud $\mathcal{P}$ via a cascaded network of PointNet~\cite{charles2017pointnet} and 3D U-Net~\cite{ronneberger2015u}.
    Our approach consists of two stages, \dan{namely} convolutional occupancy field pretraining and designed sign-agnostic, test-time implicit surface optimization.
    The former \dan{stage} is responsible \dan{for learning} the local shape priors with global consistency \dan{constraints}, and \dan{provides} relatively reasonable signed fields as \dan{initialization} for the latter \dan{stage}, \dan{which} further optimizes the whole network using the unsigned cross-entropy loss to improve the accuracy of $\mathbf{O}$. 
    \dan{We present the details of the proposed approach} in the following two sections, \ie Section~\ref{SecConvONet} and Section~\ref{SecSurfFit}.
    

\begin{figure*}[t]
    \centering
    \includegraphics[scale=0.45]{figs/pipeline.pdf}
    \vspace{0.1cm}
    \caption{\textbf{Method Overview.}   
    Our approach is built \dan{upon} the convolutional occupancy networks (CONet)~\cite{peng2020convolutional} (middle) that predicts an occupancy field $\mathbf{O}$ based on convolutional features $\mathbf{V}$ extracted from the input point cloud $\mathcal{P}$ via a cascaded network of PointNet and 3D U-Net.
    We \dan{first} pre-train the CONet~\cite{peng2020convolutional} on the accessible datasets with ground-truth $\hat{\mathbf{O}}$ using the standard binary cross-entropy (BCE) loss (top). During inference, the proposed sign-agnostic optimization further \dan{fine-tunes} the whole network parameters via unsigned cross-entropy (UCE) loss to improve the accuracy of $\mathbf{O}$ (bottom). }
    % Our approach consists of two stages, including convolutional occupancy field pretraining (top, orange) and designed signed-agnostic implicit surface optimization during inference (bottom, blue).  The  former utilizes the ground-truth occupancy fields from accessible datasets to pre-train the whole network using the standard binary cross-entropy (BCE) loss is  responsible  to  learn  the  local shape priors with global consistency constraint and provide relatively good signed fields as initializations for the latter.   The  latter  further optimize  the  whole  network  using the unsigned cross-entropy (UCE) loss to improve the accuracy of $\mathbf{O}$
    %During inference, since the pre-trained model naturally ensures global consistency and provides relatively good initialization, 
    
    \label{fig:pipeline}
    \vspace{-0.5cm}
\end{figure*}


\subsection{Convolutional Occupancy Fields Pre-training}
\label{SecConvONet} 
    
    \subsubsection{Convolutional Feature Learning}
    \label{SecUNet} 
    As shown in Figure~\ref{fig:pipeline}, we \dan{first} process the given input $\mathcal{P}$ by a shallow PointNet~\cite{charles2017pointnet} to obtain point-wise features. Then, we convert them to volumetric features with \dan{a dimension} of $H \times W \times D$\dan{,} by encapsulating local neighborhood information within a cell. \dan{Specifically,} we integrate all point features belonging to the same voxel cell using \dan{the} average pooling.
    To integrate both global and local information, we use a 3D-UNet to process $\mathbf{V}_0$ to obtain $\mathbf{V}$. Due to the \dan{issue of memory overhead} of 3D-CNN, we set $H=W=D=64$\dan{, and} the depth of the 3D U-Net is set to 4 such that the receptive field is equal to the size of $\mathbf{V}_0$.  
    \dan{Due to} the \dan{translation} equivariance of convolution operations and rich shape features integrated by the hourglass \dan{netowork architecture,} U-Net, we can enable scalable surface reconstruction for large-scale scenes. 
    
    \subsubsection{Occupancy Field Predicting}
    \label{SecOccPred} 
    Based on the obtained volumetric features $\mathbf{V}$, we can predict the occupancy probability $\mathbf{O}({\mathbf{q}}) \in \mathbb{R}^3$ of a point $\mathbf{q}$ randomly sampled in 3D space. To do this, we \dan{first} perform trilinear interpolation to query the feature vector $\mathbf{f_q}$ from $\mathbf{V}$ according to the coordinate of $\mathbf{q}$, and then feed $\mathbf{q}$ and $\mathbf{f_q}$ into the occupancy decoder $g$ that is implemented as a light-weight network of multi-layer perceptron (MLP):
    \begin{equation}
    \label{EqnOccPred}
        \mathbf{O}({\mathbf{q}})  = \mathrm{sigmoid}\left( g(\mathbf{q}, \mathbf{f_q}) \right) \in (0, 1),
    \end{equation}
    where the occupancy probability of $\mathbf{q}$ is the $\mathrm{sigmoid}$ activation of final output logit $g(\mathbf{q}, \mathbf{f_q})$.
    
    \subsubsection{Loss Function}
    \label{SecLoss} 
    During training, we uniformly sample some points $\mathcal{Q}$ within the bounding volume of watertight mesh and compute their ground truth of occupancy values. And we punish the discrepancy between the predicted and \dan{the} true occupancy values by \dan{a} loss function \dan{written as}:
    
    \begin{equation}
    \label{Eqnbce}
        \mathcal{L}(\mathbf{O}, \hat{\mathbf{O}})  = {\sum_{\mathbf{q} \in \mathcal{Q}}} 
            \texttt{BCE}\left(\mathbf{O}({\mathbf{q}}), \hat{\mathbf{O}}({\mathbf{q}})\right),
    \end{equation}
    where $\texttt{BCE}(x, y) = -y \mathrm{log}x - (1-y) \mathrm{log}(1-x)$ denotes the standard binary cross-entropy.% Note that the definition of $\texttt{BCE}(x, y)$ can take values other than 0 and 1 as the input $y$, which would be helpful for defining equation \ref{EqnUsgBce}.
    
 \subsection{Sign-Agnostic Implicit Surface Optimization}
 \label{SecSurfFit}
    In the inference stage, we can directly \dan{produce} the implicit field through a single \dan{feed-forward pass}. But we may not get satisfactory results if the given inputs are out of pre-trained priors.
    In order to improve the generality to unseen shapes, one can further optimize the pre-trained model for the given input. %to fine-tune network parameters
    But we cannot apply the loss function in Equation \ref{Eqnbce} to supervise the network finetuning, because surface normals associated with \dan{observed} points are not available, which causes the unavailability of in-out fields. Although we can choose to estimate the normals from $\mathcal{P}$, the normal estimation errors would increase the difficulty of recovering clean surfaces.

    However, the requirements of normals can be avoided by sign-agnostic optimization of occupancy field learning from hourglass convolutional networks.
    According to SAL~\cite{atzmon2020sal}, we know that by properly initializing network parameters, the implicit decoder can represent the signed field of a unit sphere, which helps us obtain signed solutions by unsigned learning objectives.
    Similarly, the pre-trained occupancy decoder can produce signed fields as \dan{initialization} for the test-time optimization. As such, we can directly employ the unsigned cross-entropy loss to \dan{obtain consistency constraints} between the occupancy field and unsigned inputs\dan{,} without the use of surface normals. Besides, global consistency \dan{among} local geometries can \dan{always be} enforced during the optimization stage, because the \dan{features} from $\mathbf{V}$ are decoded from the same global features. Thus, without the guidance of normals,  \tang{we can still guarantee globally consistent local field assemblies}.
    \dan{Specifically}, the unsigned cross-entropy (UCE) loss \dan{is} formulated as:
    \begin{equation}
     \label{EqnUsgBce}
        \mathcal{L}_{uce} = {\sum_{\mathbf{q} \in \mathcal{Q}}} 
            \texttt{BCE}\left(\mathbf{O}^{\dag}({\mathbf{q}}), \hat{\mathbf{O}}^{\dag}({\mathbf{q}})\right),
    \end{equation} 
    where prediction $\mathbf{O}^{\dag}({\mathbf{q}})$ and target $\hat{\mathbf{O}}^{\dag}({\mathbf{q}})$ are given by
    \begin{equation}
    \label{EqnAbsOcc}
        \mathbf{O}^{\dag}({\mathbf{q}}) = \mathrm{sigmoid} \big( | g(\mathbf{q}, \mathbf{f_q}) | \big) \in [0.5, 1),
    \end{equation}
    \begin{equation}
    \label{EqnUsgGT}
        \hat{\mathbf{O}}^{\dag}({\mathbf{q}}) = 
                        \left\{
                            \begin{aligned}
                                 0.5, \hspace{5pt} & \textrm{for} \ \mathbf{q} \in \mathcal{Q}_{\hat{\mathcal{S}}} \\
                                 1.0, \hspace{5pt} & \textrm{for} \ \mathbf{q}\in \mathcal{Q}_{\backslash {\hat{\mathcal{S}}}}
                            \end{aligned}
                        \right.
        ,
    \end{equation}
    % $H(x, y) = -x \textrm{log}(y)$ is discrete cross-entropy, and 
    %we can improve its generality to unseen point cloud while maintaining its learned priors as much as possible in this manner.
    where $\mathcal{Q}_{\hat{\mathcal{S}}}$ is \dan{a} point set \dan{obtained} from \dan{the} ground-truth surface $\hat{\mathcal{S}}$, and $\mathcal{Q}_{\backslash {\hat{\mathcal{S}}}}$ is \dan{a} point set sampled from non-surface volume $\mathcal{Q} \setminus \hat{\mathcal{S}}$. As $\hat{\mathcal{S}}$ is unknown at the test phase, we consider the observed surface $\mathcal{P}$ as an approximation of $\hat{\mathcal{S}}$, and identify randomly sampled points in 3D space as  non-surface points $\mathcal{Q}_{\backslash \mathcal{S}}$.
    More specifically, we  force the observed surface $\mathcal{P}$ to align with the 0.5 level set of occupancy field, and the signed occupancy values of non-surface points to be either 0 or 1.
    
    After the \dan{sign-agnostic optimization of the} implicit field, we apply the Multiresolution IsoSurface Extraction (MISE)~\cite{mescheder2019occupancy} and marching cubes~\cite{lorensen1987marching} to extract surface meshes as \dan{the} final reconstruction results. 


==> ICCV2021 Sign Agnostic ConvONet/conclusion.tex <==
\section{Conclusion}
 For the task of surface reconstruction from un-oriented point clouds, we have proposed a simple yet effective solution of learning implicit surface reconstructions by sign-agnostic optimization of convolutional occupancy networks, \tang{which achieves scalability to large scenes, generality to novel shapes, and applicability to real-world scans in a unified framework. The characteristics of implicit field learning from convolutional features of hourglass networks} enable the test-time optimization without the use of surface normals.
 %the optimization of the desired iso-surface with unsigned objectives, which avoids the use of surface normals.
 Extensive experiments on both object-level and scene-level datasets show that our method significantly outperforms the existing methods, both quantitatively and qualitatively.
 %\dan{A light practical} 
 A limitation of our approach is the slow inference speed, which is also a common drawback of test-time optimization methods. We leave it as our future effort.


==> ICCV2021 Sign Agnostic ConvONet/egpaper_final_supple.tex <==
\section*{Appendix}
In this supplementary material, we provide more details about our network \dan{architecture} in Section~\ref{SecNet}. Then we present ablation studies to validate the effectiveness of each design in our approach in Section~\ref{SecAbla}. \dan{In the next}, we demonstrate the generalization capabilities of our approach to novel categories that are different from the training category (``chair'') in Section~\ref{SecGen}. Finally, we show more qualitative \dan{comparison} with other competitive methods on the real-world \dan{3D} scene datasets in Section~\ref{SecReal}.

\section{Network Architectures}
\label{SecNet}
        \begin{figure*}[t]
        \centering
        \includegraphics[scale=0.46]{figs_supple/pointnet.pdf}
        \caption{\textbf{ResNet~\cite{he2016deep} variants of PointNet\cite{charles2017pointnet}}. It utilizes a stack of five ResNet-FC blocks with skip connections and grid-pooling layers to extract point-wise features $\mathbf{F_0}$ from the observed surface point cloud $\mathcal{P}$.}
    \label{fig:pointnet}
    \end{figure*}
    
    \begin{figure*}[t]
    \vspace{2pt}
        \centering
        \includegraphics[scale=0.48]{figs_supple/unet.pdf}
        \caption{\textbf{3D U-Net.} To effectively fuse the global and local information of input shape, we transform $\mathbf{V}_0$ (produced from $\mathbf{F}_0$) to $\mathbf{V}$ using a 3D U-Net, which consists of a series of 3D down- and up-sampling convolutions with skip connections.}
    \label{fig:unet}
    \vspace{2pt}
    \end{figure*}
    
    \begin{figure}[h]
        \centering
        \includegraphics[scale=0.52]{figs_supple/decoder.pdf}
        \caption{\textbf{Occupancy Decoder.} It contains five ResNet-FC blocks with skip connections. Given a point $\mathbf{q}$ randomly sampled in the 3D space, we query a feature vector $\mathbf{f_q}$ from the feature volume $\mathbf{V}$ according to the location of $\mathbf{q}$. Then we pass $\mathbf{q}$ and $\mathbf{f_q}$ into the occupancy decoder to predict the occupancy probability of $\mathbf{q}$ (\ie $\mathbf{O_q}$).}
    \label{fig:decoder}
    \end{figure}

    \noindent \textbf{PointNet}: The detailed network architecture of PointNet used in the paper is depicted in Figure~\ref{fig:pointnet}. Firstly, we map the coordinates of $\mathcal{P}$ into the feature space using a fully-connected (FC) layer and a ResNet-FC~\cite{he2016deep} block. Then, instead of using a global pooling operation to obtain a global feature like~\cite{charles2017pointnet}, we perform the grid-pooling operation~\cite{liao2018deep} to locally fuse the extracted features. Specifically, we perform an average-pooling operation for the features that are within the same voxel cell from a volumetric grid with the size of $64^3$. Next, we concatenate the locally pooled features with the features before pooling, and then feed the formed features into the subsequent ResNet-FC block. Overall, we use 5 ResNet blocks with intermediate grid-pooling layers to obtain the point-wise features $\mathbf{F}_0$.
    
    \noindent \textbf{3D U-Net}: The network architecture of 3D-UNet is illustrated in Figure~\ref{fig:unet}. The 3D U-Net~\cite{ronneberger2015u} is used to aggregate both local and global information of the volumetric feature $\mathbf{V}_0$ that is transformed from $\mathbf{F}_0$. The dimensions of input and output features are both set to 64. To ensure that the receptive field is equal to or larger than the size of the input feature volume, the depth of the 3D U-Net is set to 4. 
    
    \noindent \textbf{Occupancy Decoder}: As shown in Figure~\ref{fig:decoder}, the occupancy decoder consists of 5 stacked ResNet-FC blocks with skip connections. And the hidden feature dimension is set to 32.

\section{Ablation studies}
\label{SecAbla}
    
    \begin{figure}[t]
        \vspace{5pt}
        \centering
        \includegraphics[scale=0.51]{figs_supple/ablation.pdf}
        
        \begin{tabular}{p{80pt}p{80pt}p{80pt}}
            \hspace{0.3cm} (a) & \hspace{0.4cm} (b) &\hspace{0.4cm} (c)
        \end{tabular}
        \caption{\textbf{Additional Qualitative Ablation Studies:} (a) input point clouds, (b) without the pre-training of convolutional occupancy networks, and (c) Ours.}
    \label{fig:ablation}
    \end{figure}
    In this section, we conduct additional ablation studies by alternatively removing one of the modules of the proposed approach to verify the effectiveness of them.
    
    % \noindent \textbf{without the pre-training of convolutional occupancy networks (w/o pre-training)}
\noindent \textbf{Effect of pre-training (\ie~w/o pre-training)}
    Based on our approach, an alternative solution to provide \dan{initialization of the} signed field for the proposed sign-agnostic optimization is to adopt the geometric initialization as in SAL~\cite{atzmon2020sal}, which initializes the implicit decoder to approximate the signed distance field of the unit sphere. The visualization comparisons are shown in Figure~\ref{fig:ablation}. Without the pre-trained shape prior, the sign agnostic optimization fails to reconstruct reasonable geometries.

    \noindent \textbf{Effect of only optimizing the encoder (\ie~opt. enc.)} In all experiments, we choose to optimize the whole network parameters with the unsigned binary cross-entropy loss during inference. An alternative solution is to only optimize the encoder (\ie~PointNet and 3D U-Net) while freezing the occupancy decoder. The comparisons shown in Table~\ref{table:ablation}  clearly demonstrate that jointly optimizing the whole network can achieve better generality to unseen shapes.
    
    \input{tabs_supple/ablation.tex}
    
    \noindent\textbf{Ablation studies on the iteration number of the test-time optimization.} Fig.~\ref{fig:vary_iter:quanti} and~\ref{fig:vary_iter:quali} show the quantitative and qualitative results w.r.t. the number of iterations, respectively. {Notably, the `Iter 0' represents the result before optimization.} We can observe that after about 600 iterations of the test-time optimization, the results become stable.
    
    \begin{figure}[h]
        %\vspace{-8pt}
    	\centering
    	\includegraphics[width=1.0\linewidth]{figs_supple/vary_iter_quanti2.png}
    	\caption{Quantitative results obtained at different iterations during the test-time optimization. {Experiments are conducted on the synthetic room dataset with the input of 30,000 points.}}
    	%\vspace{-0.3cm}
    	\label{fig:vary_iter:quanti}
    \end{figure}
    
    \begin{figure}[h]
        %\vspace{-5pt}
    	\centering
    	\includegraphics[width=1.0\linewidth]{figs_supple/vary_iter_qualita.pdf}
    	\caption{Examples of qualitative results of {a synthetic room} obtained at different iterations during the test-time optimization.}
    	%\vspace{-0.2cm}
    	\label{fig:vary_iter:quali}
    \end{figure}

    \noindent\textbf{Ablation studies on the sparsity level of the input.} Quantitative results for different sparsity levels of the input are shown in Table~\ref{table:sparsity:chair} and ~\ref{table:sparsity:synthetic_room}. We can observe that the results of different evaluation metrics only show a slightly small variance, which clearly demonstrates the robustness of our method against the input sparsity.
    
    \input{tabs_supple/ablation_sparsity.tex}

\section{Novel Categories Generalization}
\label{SecGen}
    \begin{figure*}[t]
    \vspace{5pt}
        \centering
        %\vspace{-5pt}
        \includegraphics[scale=0.128]{figs_supple/novelcat.pdf}
        
        \begin{tabular}{p{60pt}p{53pt}p{53pt}p{53pt}p{53pt}p{53pt}p{53pt}p{53pt}}
                 \ \ Input PC  & 
                 \  SPSR \cite{kazhdan2013screened} &
                 \ ONet \cite{mescheder2019occupancy} & 
                 \  SAL \cite{atzmon2020sal}  & 
                 \ IGR \cite{gropp2020implicit} & 
                 \ CONet \cite{peng2020convolutional}  &
                 \ \ \ LIG \cite{jiang2020local} &  
                 \ Ours
        \end{tabular}
        \caption{\textbf{Generalize to Novel Categories.} We directly evaluate our approach and baselines on unseen, novel categories including ``bench'', ``lamp'', and ``watercraft'' that are very different from the training ``chair'' category.}
    \label{fig:novelcat}
    \end{figure*}
    In this section, we analyze the generalization performance of our approach and the baselines on the object-level reconstruction. We directly evaluate them on novel categories such as ``bench'', ``lamp'' and ``watercraft'' that are different from the training ``chair'' category. As shown in Figure~\ref{fig:novelcat}, our approach can preserve more geometric details such as small holes, long rods, and thin parts, while the baselines cannot. This demonstrates the superior generalization capabilities of the proposed approach to unseen categories.


\section{Real-world Scenes Generalization}
\label{SecReal}
    In this section, we \dan{first} describe the implementation details of sign-agnostic optimization of convolutional occupancy networks in a sliding-window manner, and then provide more qualitative \dan{comparison} on the real-world scenes \dan{datasets including} ScanNet-V2~\cite{dai2017scannet} and Matterport3d~\cite{chang2017matterport3d}.
    
    %\noindent \textbf{Implementation Details of Sign-Agnostic Optimization in a Sliding-window Manner.}
    \subsection{Implementation Details of Sign-Agnostic Optimization in a Sliding-Window Manner}
    In the experiments of object-level and synthetic scene reconstruction, we perform pre-training and sign-agnostic optimization within the unit cube. However, this strategy cannot deal with real-world scenes that are arbitrarily sized and represented in meters.
    Although we can resize these scenes into the unit cube, convert them into volumetric grids of size $64^3$, and then process them using the 3D U-Net as described in Section~\ref{SecNet}, we may not be able to recover fine-grained geometries as the low-resolution voxelization process loses much information about surface details, while the high-resolution voxelization such as $128^3, 256^3$ would suffer from the heavy computation cost and memory issues.
    Thanks to the \dan{translation equivalence} of fully convolutional networks, we can apply the proposed model to local patches cropped from large scenes and perform implicit surface reconstruction in a sliding-window manner, which can help us preserve the input information while avoiding memory issues of 3D CNNs.
    
    More specifically, we also pre-train our model on the synthetic indoor scene dataset~\cite{peng2020convolutional} where the size of scenes is approximately a real-world unit of 4.4m $\times$ 4.4m $\times$ 4.4m. Similar to the setting of~\cite{peng2020convolutional}, we set the voxel size as 0.02m such that each scene is contained in a volumetric grid with size $220^3$. 
    During the network pre-training, we utilize the Res-PointNet and 3D U-Net described in Section~\ref{SecNet} to learn corresponding convolutional features from each cropped subvolume. Then we predict the occupancy probabilities of query points uniformly sampled from the grid of input subvolume. 
    Specifically, we randomly sample one point within the whole scene and use it as the center of the subvolume. 
    The size of each cropped subvolume~(\ie $H \times W \times D$) is set to $25 \times 25 \times 25$. 
    Since the receptive field of 3D U-Net is 64, we set the size of input subvolumes to $(H + 63) × (W + 63) + (D + 63) = 88 \times 88 \times 88$. At each iteration, we use a batch size of 4 subvolumes.
    
    During the test-optimization stage, we divide the large scene into overlapped subvolumes and then perform sign-agnostic optimization for each subvolume in a sliding-window manner. We determine the size of cropped subvolumes according to the size of input scenes such that they are compatible with the GPU memory. Notably, we do not need the padding operation as the cropped subvolumes overlap.
    
    %\noindent \textbf{Additional Qualitative Comparisons.}
    \subsection{Additional Qualitative Results}
    We have provided more qualitative comparisons on the ScanNet~\cite{dai2017scannet} in Figure~\ref{fig:scannet_fig2}.
    Besides, more visualized results on the Matterport3D~\cite{chang2017matterport3d} are shown in Figure~\ref{fig:matterport_fig1}. 
    From these results, we can clearly observe that our method achieves more superior performance to large scenes with multiple rooms than the existing state-of-the-arts.
    And in comparison with those baselines such as SPSR~\cite{kazhdan2013screened, jiang2020local} that heavily rely on accurate surface normals, our approach can avoid the degenerated results caused by inaccurate normal estimation. Besides, compared to CONet~\cite{peng2020convolutional}, our approach can reconstruct more complete geometries and preserve complicated geometric details well, which validates the effectiveness of the proposed sign-agnostic optimization during inference. Overall, our method simultaneously maximizes the scalability to large scenes, generality to unseen shapes, and applicability to real scans that lack reliable surface normals.

    % \begin{figure*}[t]
    %     \begin{tabular}{cc}
    %       \rotatebox[origin=c]{90}{
    %         \begin{tabular}{c c c c c c}
    %         \quad \quad GT \quad \quad \quad \quad \quad \quad  \quad &
    %             Ours \quad \quad \quad \quad \quad \quad  & 
    %             LIG\cite{jiang2020local} \quad \quad \quad \quad \quad  \quad \quad &
    %             CONet\cite{peng2020convolutional} \quad \quad \quad  \quad \quad  & 
    %             SPSR\cite{kazhdan2013screened} \quad \quad \quad \quad \quad & 
    %             Input PC \quad \quad \quad 
    %         \end{tabular}
    %         } & 
    %       \hspace{-0.5cm}
    %       \raisebox{-.5\height}{\includegraphics[scale=0.165]{figs_supple/scannet_fig1.pdf}}
    %     \end{tabular}
    
    % \begin{tabular}{p{120pt}p{120pt}p{120pt}p{120pt}}
    % \hspace{3.0cm} (a) & \hspace{2.5cm} (b) & \hspace{1.8cm} (c) & \hspace{0.9cm} (d)
    % \end{tabular}
    %     \caption{\textbf{Scene-level Reconstruction on ScanNet~\cite{dai2017scannet}.} Qualitative comparisons for surface reconstruction from un-orientated scans of ScanNet. All methods except SPSR are trained on the synthetic room dataset and directly evaluated on ScanNet.}
    %     \label{fig:scannet_fig1}
    % \end{figure*}
    
    \begin{figure*}[t]
        \begin{tabular}{cc}
          \rotatebox[origin=c]{90}{
            \begin{tabular}{c c c c c c}
            \quad \quad GT \quad \quad \quad \quad \quad \quad  \quad &
                Ours \quad \quad \quad \quad \quad \quad  & 
                LIG\cite{jiang2020local} \quad \quad \quad \quad \quad  \quad \quad &
                CONet\cite{peng2020convolutional} \quad \quad \quad  \quad \quad  & 
                SPSR\cite{kazhdan2013screened} \quad \quad \quad \quad \quad & 
                Input PC \quad \quad \quad 
            \end{tabular}
          } & 
          \hspace{-0.5cm}
          \raisebox{-.5\height}{\includegraphics[scale=0.165]{figs_supple/scannet_fig2.pdf}}
        \end{tabular}
    
    \begin{tabular}{p{120pt}p{120pt}p{120pt}p{120pt}}
    \hspace{3.0cm} (a) & \hspace{2.5cm} (b) & \hspace{1.8cm} (c) & \hspace{0.9cm} (d)
    \end{tabular}
        \caption{\textbf{Scene-level Reconstruction on ScanNet~\cite{dai2017scannet}.} Qualitative comparisons for surface reconstruction from un-orientated scans of ScanNet. All methods except SPSR are trained on the synthetic room dataset and directly evaluated on ScanNet.}
        \label{fig:scannet_fig2}
    \end{figure*}
    
    \begin{figure*}[t]
        \begin{tabular}{cc}
          \rotatebox[origin=c]{90}{
            \begin{tabular}{c c c c c c}
            \quad GT \quad \quad \quad \quad \quad \quad \quad &
                Ours \quad \quad \quad \quad \quad \quad \quad & 
                LIG\cite{jiang2020local} \quad \quad \quad \quad \quad \quad& 
                CONet\cite{peng2020convolutional} \quad \quad \quad \quad \quad \quad& 
                SPSR\cite{kazhdan2013screened} \quad \quad \quad \quad \quad & 
                Input PC 
            \end{tabular}
          } & 
          \hspace{-0.5cm}
          \raisebox{-.5\height}{\includegraphics[scale=0.165]{figs_supple/matterport_fig1.pdf}}
        \end{tabular}
    
    \begin{tabular}{p{200pt}p{200pt}}
    \hspace{3.0cm} (a) & \hspace{3.5cm} (b) 
    \end{tabular}
        \caption{\textbf{Scene-level Reconstruction on Matterport 3D~\cite{chang2017matterport3d}.} Qualitative comparisons for surface reconstruction from un-orientated scans of  Matterport3D. All methods except SPSR are trained on the synthetic room dataset and directly evaluated on Matterport 3D.}
        \label{fig:matterport_fig1}
    \end{figure*}
    
    % \begin{figure*}[t]
    %     \begin{tabular}{cc}
    %       \rotatebox[origin=c]{90}{
    %         \begin{tabular}{cccccc}
    %         \quad GT \quad \quad \quad \quad \quad \quad \quad &
    %             Ours \quad \quad \quad \quad \quad \quad \quad & 
    %             LIG\cite{jiang2020local} \quad \quad \quad \quad \quad \quad& 
    %             CONet\cite{peng2020convolutional} \quad \quad \quad \quad \quad \quad& 
    %             SPSR\cite{kazhdan2013screened} \quad \quad \quad \quad \quad & 
    %             Input PC \quad \quad 
    %         \end{tabular} 
    %       } & 
    %       \hspace{-0.5cm}
    %       \raisebox{-.5\height}{\includegraphics[scale=0.165]{figs_supple/matterport_fig2.pdf}}
    %     \end{tabular}
    
    % \begin{tabular}{p{200pt}p{200pt}}
    % \hspace{3.0cm} (a) & \hspace{3.5cm} (b) 
    % \end{tabular}
    %     \caption{\textbf{Scene-level Reconstruction on Matterport 3D~\cite{chang2017matterport3d}.} Qualitative comparisons for surface reconstruction from un-orientated scans of  Matterport 3D. All methods except SPSR are trained on the synthetic room dataset and directly evaluated on Matterport 3D.}
    %     \label{fig:matterport_fig2}
    % \end{figure*}

==> ICCV2021 Sign Agnostic ConvONet/experiment.tex <==
\section{Experiments}
\label{SecExp}

\noindent \textbf{Datasets} We validate the \dan{efficiency} of our method on experiments of both object-level and scene-level surface reconstruction \dan{tasks}. For the former \dan{task}, we conduct \dan{comparison} on the \emph{chair} category of \dan{the} ShapeNet~\cite{chang2015shapenet} dataset. %, due to their complex topologies and surface details
For the latter \dan{task}, we use the synthetic indoor scene dataset ~\cite{peng2020convolutional}.
The split of train/val/test sets \tang{follows} the same setting in  CONet~\cite{peng2020convolutional}. For each dataset, we randomly select 50 models from the test set to conduct quantitative evaluations.
 We use point clouds of size 30, 000 sampled from true surfaces as inputs. Finally, we compare the synthetic-to-real generality by conducting experiments on ScanNet-V2~\cite{dai2017scannet} and Matterport3D~\cite{chang2017matterport3d} datasets.

\noindent \textbf{Implementation Details}  
%Following~\cite{mescheder2019occupancy, peng2020convolutional}, 
We \dan{first} pre-train the convolutional occupancy networks \dan{with} a batch size of 32 and \dan{a} learning rate of $1 \times 10^{-4}$ for \dan{overall} 300k iterations.
During the sign-agnostic optimization, the whole network is further optimized by the objective \dan{described} in Equation~\ref{EqnUsgBce} using a batch size of 16 for 1000 iterations. The initial learning rate is set to $3 \times 10^{-5}$, and decays by 0.3 every 400 iterations.
We set $|\mathcal{Q}_{\hat{\mathcal{S}}}| = 512$ and $|\mathcal{Q}_{\backslash {\hat{\mathcal{S}}}}| = 1,536$ in Equation~\ref{EqnUsgGT}.

\noindent \textbf{Baselines}
We conduct \dan{comparison} with three categories of existing methods, \dan{i.e.} classic optimization-based methods such as Screened Poisson Surface Reconstruction (SPSR)~\cite{kazhdan2013screened},
deep optimization-based methods such as Sign-Agnostic Learning (SAL)~\cite{atzmon2020sal} and Implicit Geometric Regularization (IGR)~\cite{gropp2020implicit},
learning-based methods such as Occupancy Networks (ONet)~\cite{mescheder2019occupancy} and Convolutional Occupancy Networks (CONet)~\cite{peng2020convolutional}, 
\dan{and} methods \dan{focusing on} optimizing data-driven \dan{priors} such as Local Implicit Grid (LIG)~\cite{jiang2020local}. For SAL and IGR, we directly fit the neural implicit field to the observed point cloud. For ONet, CONet, and LIG, the evaluations are based on their provided pre-trained models.
\dan{Specifically,} we summarize their respective characteristics in Table \ref{table:compare_chara}. For methods that require oriented surface normals, we follow~\cite{hoppe1992surface} to estimate un-oriented normals and then reorient their directions.
% ONet, SAL, and IGR focus on global shape learning, while  CONet, LIG, and our method perform local geometry reasoning.

\input{tabs/method_compara.tex}


\noindent \textbf{Evaluation Metrics}
%Intersection-over-Union (IoU),
We consider Chamfer Distance (CD $\times 0.01$), Normal Consistency (NC $\times 0.01$), and F-score (FS $\times 0.01$) as primary evaluation metrics. The F-score is reported with thresholds of $\tau$ and $2\tau$ ($\tau = 0.01$).
\dan{The} quantitative results between two point clouds are measured from randomly sampled ten thousand surface points. For the CD, the lower is better. For NC and FS, the higher is better.

\section{Object-level Reconstruction}
\label{SubSecExpObj}
      \input{tabs/chair.tex}
    
    \begin{figure*}[!htb]
            %\vspace{-6pt}
            \centering 
            \includegraphics[scale=0.135]{figs/chair.pdf}
                \begin{tabular}{p{60pt}p{53pt}p{53pt}p{53pt}p{53pt}p{53pt}p{53pt}p{53pt}}
                 \quad \quad Input PC  & 
                 \quad SPSR \cite{kazhdan2013screened} &
                 \quad ONet \cite{mescheder2019occupancy} & 
                 \quad SAL \cite{atzmon2020sal}  & 
                 IGR \cite{gropp2020implicit} & 
                 CONet \cite{peng2020convolutional}  &
                 LIG \cite{jiang2020local} &  
                 Ours
                \end{tabular}
                %\vspace{-5pt}
                \caption{\textbf{Object-level Reconstruction on ShapeNet.} Qualitative \dan{comparison} for surface reconstruction from un-orientated point clouds of ShapeNet-chair~\cite{dai2017scannet}.}
                \label{fig:chair}
            
    \end{figure*}
    
    
    \begin{figure*}[!htb]
            %\vspace{-6pt}
            \centering 
                \includegraphics[scale=0.127]{figs/synroom.pdf}
                \begin{tabular}{p{62pt}p{62pt}p{62pt}p{62pt}p{62pt}p{62pt}p{62pt}}
                     \quad Input PC & 
                     \quad SPSR \cite{kazhdan2013screened} &
                     \quad SAL \cite{atzmon2020sal}  & 
                     IGR \cite{gropp2020implicit} & 
                     CONet \cite{peng2020convolutional}  &
                     LIG \cite{jiang2020local} &  
                     Ours
                    \end{tabular}
                %\vspace{-5pt}
                \caption{\textbf{Scene-level Reconstruction on synthetic rooms.} Qualitative \dan{comparison} for surface reconstruction from un-orientated point \dan{clouds} on the synthetic room indoor scene dataset provided by~\cite{peng2020convolutional}.}
                \label{fig:synroom}
    \end{figure*}
    
    We \dan{first} conduct the object-level reconstruction experiments. 
    To \dan{simulate} the influence of sensing noises during real scans acquisition, we perturb 
    the input by gaussian noise with zero mean and standard deviation 0.05.
    
    As shown in Figure~\ref{fig:chair},  our approach has demonstrated superiority in terms of visual quality in the complex object reconstruction.
    Compared to the methods of only using global shape features such as ONet~\cite{mescheder2019occupancy}, SAL~\cite{atzmon2020sal}, and IGR~\cite{gropp2020implicit}), ours \dan{is} more capable of recovering complicated geometries because we utilize rich shape features, including \dan{both} local \dan{and} global information. Besides, instead of strictly respecting the learned \dan{priors} like CONet~\cite{peng2020convolutional}, more faithful surface details (e.g. slender bars and tiny holes) can be preserved by breaking the barrier of pre-trained \dan{priors} during inference.
    In addition, SPSR~\cite{kazhdan2013screened}, IGR~\cite{gropp2020implicit}, and LIG~\cite{jiang2020local} tend to produce degenerated meshes, caused by inaccurate normal orientation estimation.  However, it has no negative effects on our results, as we do not use the additional information during the test-time optimization.
    Our superiority is also verified by numerical results reported in Table~\ref{table:chair}, where our method outperforms existing state-of-the-art methods by large margins.
    %By applying sign-agnostic optimization, our reconstructions faithfully respect the observed points and preserve fine-grained surface details (e.g. slender bars and tiny holes).

\section{Scene-Level Reconstruction}
    \input{tabs/synthetic_room.tex}
    
    To investigate whether our method possesses the scalability to indoor scene reconstructions, we \dan{further} conduct the experiments of 3D reconstruction from un-oriented point clouds on the synthetic indoor scene dataset \cite{peng2020convolutional}. 
    %Following the setting of Section \ref{SubSecExpObj}, we uniformly sample 30,000 points as input point cloud $\mathcal{P}$. 
    From the qualitative \dan{comparison shown} in Figure~\ref{fig:synroom}, we can \dan{observe} that some subtle legs of chairs can also be recovered by our approach, while others cannot capture these details. This demonstrates that ours can scale well to large scenes as we adopt the strategy of local geometry reasoning, instead of global shape modeling \dan{as} in SAL~\cite{atzmon2020sal} and IGR~\cite{gropp2020implicit}. 
    Compared to CONet~\cite{peng2020convolutional}, more fine-grained surface recoveries demonstrate that our approach can achieve better generality to novel scenes, due to the effective sign-agnostic optimization that conforms the desired implicit surface to the observed un-oriented surfaces.
    Moreover, the bypassing of normal estimation enables more robust scene-level surface reconstructions.
    Again, better quantitative results presented in Table~\ref{table:synthetic_room} consistently demonstrate the superiority of our approach. 
    %since we simultaneously achieve advanced scalability to large scenes, generality to novel shapes, and applicability to real scans in a unified framework,
    
    %\tang{Overall, our method can significantly outperform the existing methods in both object-level and scene-level reconstruction.}
    
    \input{tabs/scannet.tex}
    

\begin{figure*}[t]

    \begin{tabular}{cc}
      \rotatebox[origin=c]{90}{
        \begin{tabular}{cccccc}
        \quad GT \quad \quad \quad \quad \quad \quad \quad &
            Ours \quad \quad \quad \quad \quad \quad \quad & 
            LIG\cite{jiang2020local} \quad \quad \quad \quad \quad \quad& 
            CONet\cite{peng2020convolutional} \quad \quad \quad \quad \quad \quad& 
            SPSR\cite{kazhdan2013screened} \quad \quad \quad \quad \quad & 
            Input PC 
        \end{tabular}
      } & 
      \hspace{-0.5cm}
      \raisebox{-.5\height}{\includegraphics[scale=0.165]{figs/scannet.pdf}}
    \end{tabular}

\begin{tabular}{p{120pt}p{120pt}p{120pt}p{120pt}}
\hspace{3.0cm} (a) & \hspace{2.5cm} (b) & \hspace{1.8cm} (c) & \hspace{0.9cm} (d)
\end{tabular}

    \caption{\textbf{Scene-level Reconstruction on ScanNet~\cite{dai2017scannet} and Matterport3D~\cite{chang2017matterport3d}.} Qualitative \dan{comparison} for surface reconstruction from un-orientated scans of ScanNet (a, b, c) and Matterport3D (d). All methods except SPSR are trained on the synthetic room dataset and directly evaluated on ScanNet.}
    \label{fig:scannet}
\end{figure*}



\section{Real-World Scenes Generalization}
To compare the generalization performance on real-world scans, we also evaluate our approach on the real-world datasets, including ScanNet~\cite{dai2017scannet} and Matterport3D~\cite{chang2017matterport3d}. Notably, all models are only trained on the \dan{same} synthetic indoor scene dataset. 
% Similar to previous experimental settings, we use randomly sampled points $\mathcal{P}$ of size 30,000 as input point cloud.

\noindent \textbf{ScanNet-V2} The qualitative and quantitative comparisons are respectively shown in Figure \ref{fig:scannet} and Table \ref{table:scannet}. As \dan{can be} seen, compared to other methods, our results achieve \dan{clearly} better numerical scores and \dan{more fine-grained} surface geometries, which \dan{effectively verifies} the better generalization ability of \dan{the} proposed method on real-world scans.

\noindent \textbf{Matterport3D} To evaluate its scalability to huge scenes that contain multiple rooms, we finally conduct experiments on the Matterport3D dataset~\cite{chang2017matterport3d}. Following the sliding-window strategy presented in~\cite{peng2020convolutional}, we separately apply the designed sign-agnostic optimization of convolutional occupancy networks to each room. The visualization \dan{comparison is} presented in Figure~\ref{fig:scannet} (d).
Notably, the Matterport3D~\cite{chang2017matterport3d} is significantly different from the synthetic indoor room dataset that is used to pre-train our network. But our reconstruction results can still preserve rich details inside each room while adhering to the room layout, which \dan{fully} demonstrates that our method can achieve better scalability to huge scenes and better robustness to noises from \dan{different} sensing devices.

%enables us to reconstruct scenes at any scale




==> ICCV2021 Sign Agnostic ConvONet/introduction.tex <==
\section{Introduction}
\label{SecIntro}
    Surface reconstruction from point clouds is of significance to perceive and understand surrounding 3D worlds for intelligent systems, which plays a \dan{fundamental} role in numerous practical applications, such as computer-aided design, 3D printing, and robotics grasping. Recently, this problem has attracted \dan{wide} attention as inexpensive and portable commodity scanners such as the Microsoft Kinect make it much easier to acquire 3D point clouds. Classical methods~\cite{alexa2003computing, carr2001reconstruction, levin2004mesh, kazhdan2006poisson, kazhdan2013screened} \dan{tackle} this problem by mathematical optimization according to pre-defined geometric priors, while learning-based methods ~\cite{groueix2018atlasnet, chibane2020implicit, mescheder2019occupancy, peng2020convolutional} choose to learn geometric priors from large-scale 3D datasets in a data-driven manner. %, which demonstrate better robustness than classic methods. 
    Recently, \dan{representing 3D surface as an implicit field} has gained \dan{large} popularity~\cite{chen2019learning, mescheder2019occupancy, park2019deepsdf, saito2019pifu, xu2019disn, chibane2020implicit, jiang2020local, chabra2020deep, erler2020points2surf, tretschk2020patchnets, peng2020convolutional, tang2021skeletonnet}. Compared to other shape representations \dan{such as} voxel~\cite{choy20163d, wu2016learning}, octree~\cite{riegler2017octnet, tatarchenko2017octree, wang2018adaptive, hane2017hierarchical}, point cloud~\cite{fan2017point} and mesh~\cite{groueix2018atlasnet, wang2018pixel2mesh, kato2018neural, tang2019skeleton, pan2019deep, tang2021skeletonnet}, continuous implicit fields can enable surface reconstruction with infinite resolution and arbitrary topology. 
    
    A lot of methods have been proposed to \dan{advance} the development of implicit surface reconstruction from various respects in terms of improving scalability, generality, and applicability. \dan{However,} there is still not an approach \dan{in the literature} to simultaneously achieve all these \dan{objectives with satisfactory performance}.
    Targeting better scalability \tang{to} large-scale scenes, \dan{several} approaches~\cite{jiang2020local, chabra2020deep,  tretschk2020patchnets, peng2020convolutional, erler2020points2surf} learn local implicit fields and model a global shape as a composition of local surface geometries, rather than conducting global shape reasoning from a latent code.
    \dan{Towards} better generality \tang{to} novel shapes, \dan{some works}~\cite{park2019deepsdf, gropp2020implicit,jiang2020local, chabra2020deep, tretschk2020patchnets, yang2020deep} attempt to optimize the pre-trained priors at test time to \tang{obtain a better} solution for each given input, instead of strictly respecting the learned priors. 
    Existing state-of-the-art methods~\cite{jiang2020local, chabra2020deep, tretschk2020patchnets} improve both scalability and generality \dan{via individual optimization of } each local implicit field during inference.
    However, without explicitly considering geometric relationships between local fields,
    they heavily rely on accurate normals to avoid the sign conflict problems in the overlapped regions of local fields.  
    Although SAL~\cite{atzmon2020sal} breaks this limitation via sign-agnostic learning that improves the applicability to real-world scans where surface normals are unavailable, it can only perform global shape modeling. \tang{Further works still need to explore how to extend this technique for local shape modeling.}
    
    To this end, we propose to learn implicit surface reconstructions by sign-agnostic optimization of convolutional occupancy networks~\cite{peng2020convolutional}, to simultaneously achieve \dan{the three important reconstruction objectives,} \ie~advanced generality, specialty, and applicability in a unified framework. \dan{We achieve} this goal by a simple yet effective solution that further optimizes the pre-trained occupancy prediction networks via sign-agnostic learning. The learning of occupancy fields is conditioned on convolutional features from an hourglass network (\eg~U-Net~\cite{ronneberger2015u}).
    Our solution is motivated by two key characteristics.
    The first characteristic is that, after being pre-trained on the accessible datasets with ground-truth signed fields, the occupancy decoder can provide a signed field as initialization for the test-time optimization. Thus we can further apply unsigned objectives to optimize occupancy prediction networks, maximizing the consistency between the desired iso-surface with the observed un-oriented point cloud.
    The second characteristic is that, the U-Net~\cite{ronneberger2015u} aggregates both local and global information in an hourglass convolutional manner. The use of local shape features not only preserves the fine-grained geometries, but also enables the surface recovery of large-scale indoor scenes.
    The integrated global shape features can enforce geometric consistency between learned local geometries and guarantee the assembly of local fields as a globally consistent one, \dan{although} we do not \dan{utilize} guidance from additional normal information.
    As shown in Figure~\ref{fig:teaser}, we can reconstruct surfaces with \dan{fine} details directly from un-oriented point clouds \emph{without the use of normals}, \dan{for both} complicated objects to large-scale scenes.
    % \par The main contribution can be summarized as follow:
    % \begin{itemize}
    %     \item{We simultaneously achieve \dan{reconstruction objectives of} advanced scalability, generality, and applicability in a unified framework,  which enables robust object-level and scene-level surface reconstruction with high-fidelity details from un-oriented point clouds.}
    %     \item{We propose a simple yet effective solution of learning implicit surface reconstruction by sign-agnostic optimization of convolutional occupancy networks.}
    % \end{itemize}
    
    Extensive \dan{experimental} comparisons \dan{with} state-of-the-arts on both object-level and scene-level datasets, including ShapeNet~\cite{chang2015shapenet}, synthetic indoor scene dataset~\cite{peng2020convolutional}, and real-world scene datasets (ScanNet~\cite{dai2017scannet} and Matterport3D~\cite{chang2017matterport3d}) demonstrate the superior \dan{performance} of our approach for surface reconstruction from un-oriented point clouds. 
    
    
    %More superior performance on the real-world scene dataset including ScanNet~\cite{dai2017scannet} and Matterport3D~\cite{chang2017matterport3d} illustrate the better generalization capability of our method.
    
    %And superior results on varying point cloud sizes and noise levels indicate the robustness of our method to noise and sparsity.

==> ICCV2021 Sign Agnostic ConvONet/problem.tex <==
%%%%V0

\section{Problem Statement}
\label{SecPro}
    Given a set of observed points $\mathcal{P} = \{\bm{p}_i \in \mathbb{R}^3 \}_{i=1}^n$, the goal of our method is to reconstruct a surface $\mathcal{S}$ that is as similar as possible to the underlying surface $\hat{\mathcal{S}}$.  The problem is pretty intractable for several reasons. On one hand, it is severely ill-posed to compute a continuous surface from its discrete approximation, since there could be infinitely possible solutions. Classic optimization-based methods try to alleviate this ambiguity by pre-defined geometric priors. Recent data-driven methods choose to learn shape priors from large-scale datasets. Nonetheless, there is still no satisfactory solution. 
    Classic methods are sensitive to imperfect observations.
    Most learning-based methods strictly fix the learned prior at the test phrase~\cite{mescheder2019occupancy}, which causes the over-smoothness of high-frequent surface details.  %Global shape optimization~\cite{park2019deepsdf, gropp2020implicit} during inference usually has limited generality to large scenes, while local surface optimization requires additional normal information to enforce the global consistency of local assembly. 
    On the other hand, the inverse problem becomes even more difficult and challenging when we consider processing real scans where reliable normals are not associated with observed points. 
    %Due to imperfection of scan acquisition, the observed points could be noisy, incomplete, and irregularly distributed. Mathematically, the given point cloud $\{\bm{p}_i\}_{i=1}^n$ could be represented as $\{\bm{x}_i+\bm{\epsilon}_i\,|\,\bm{x}_i\in \hat{\mathcal{S}}\}_{i=1}^n$, with possibly perturbations $\{\bm{\epsilon}_i\}_{i=1}^n$. The noises can increase the errors of normal estimation, which increases the uncertainty of given data and thus the difficulty of recovering clean surfaces. 
    However, exiting state-of-the-arts, which individually optimize learned local implicit field during inference, heavies rely on accurate surface normals to enforce the global consistency of local assembly. 
    Thus the normal estimation errors would increase the uncertainty of given data and the difficulty of recovering clean surfaces.
    To this end, we aim to pursue a novel approach of local implicit field optimization that inherits the advantages of local field learning and optimization strategy. But we target surface reconstruction directly from un-oriented point clouds without the use of normal information. 
    

    
\section{Approach}
\label{SecApp}
    % Karbo
    % {\color{blue}Our proposed method mainly dedicate to tackle the problem of reconstructing possibly large scenes from unoriented point clouds while recovering as many geometric details as possible presented in the observations. Since our task is to obtain a signed implicit field from an unsigned point cloud, global awareness is requisite for our network to differentiate the interior of the solid objects. To this end, we adopt a trained convolutional occupancy network as our backbone. Briefly, the network forms a feature volume via integrating per-point features in a sign-agnostic manner, then processes the volume by a 3D-UNet to aggregate both the local and global information, finally extract the surface mesh from the obtained interpolated occupancy volume via marching cubes. To ensure the reconstruction faithfully presents the input observation, we adapt the learned prior encoded in the trained network via additionally optimizing the network parameters by conforming the predictions to our observed point cloud. This can be achieved by simply minimizing the unsigned binary cross-entry loss at test phase. 
    % The overall network composition will be detailed in SectionXXX. The test-optimiztion procedure will be presented in SectionXXX.}
    
    Our proposed method is primarily motivated from the characteristic of hourglass networks such as U-Net~\cite{ronneberger2015u}, which consists of a series of down- and up-sampling convolutions with skip connections to aggregate both local and global information. 
    In this way, the final output features at different spatial positions naturally respect the global shape prior, which implicitly constraint the global consistency between local fields that are learned from these features. 
    Besides, inspired by SAL~\cite{atzmon2020sal}, we resort to auxiliary datasets with occupancy field groundtruths to pre-train our model. This can initialize the occupancy decoder as a signed field before the test-optimization. 
    Thus, different from those methods ~\cite{jiang2020local, chabra2020deep, tretschk2020patchnets} that individually optimize each local field and utilize the provided orientation information to solve the sign flipping problem between local fields, we can jointly optimize local fields by optimizing the convolutional features learned in a hourglass manner without the use of surface normals. 
    This means we do not need to consider the sign flipping problem between local fields.
    we can a self-supervised objective to maximize the consistency between learned local implicit fields and input observation.
        
     The overall pipeline of our method is illustrated in Fig.\ref{fig:pipeline}. 
     We will present more details about network architecture ( Sec.~\ref{SecUNet} and Sec.~\ref{SecOccPred}), and training paradigm (Sec.\ref{SecLoss}) to learn local shape prior and pretrain the occupancy decoder as a signed field. Next we will discuss our proposed signed-agnostic implicit surface fitting during inference in the Sec.~\ref{SecSurfFit}.
     
     
     
%%%%V1

\subsection{Overview}
\label{SubSecOver}
    Given a set of observed points $\mathcal{P} = \{\bm{p}_i \in \mathbb{R}^3 \}_{i=1}^n$, the goal of our method is to reconstruct a implicit surface $\mathcal{S}$ that is as similar as possible to the underlying surface $\hat{\mathcal{S}}$.  It is severely ill-posed to compute a continuous surface from its discrete approximation, since there could be infinitely possible solutions. Classic optimization-based methods try to alleviate this ambiguity by pre-defined geometric priors. Recent data-driven methods choose to learn shape priors from large-scale datasets to improve the robustness to imperfect observations.
    {\color{red}
    A lot of methods have been proposed  to push the progress of implicit surface reconstruction from various respects, in terms of improving generality, specialty, and applicability. But there is still not an approach that can simultaneously achieve advancements in all three respects. Most learning-based methods~\cite{mescheder2019occupancy, chen2019learning, peng2020convolutional} strictly fix the learned prior during inference, resulting in the over-smoothness of high-frequency surface details.  
    Global shape optimization~\cite{park2019deepsdf, gropp2020implicit, yang2020deep} during inference usually has limited generality to large scenes, while local surface optimization~\cite{jiang2020local, chabra2020deep, tretschk2020patchnets} requires additional normal information that are not always avaiable in real scans to enforce the global consistency of local field assembly. 
    Although SAL~\cite{atzmon2020sal} bypass the requirements of normals via sign-agnostic learning, it can only work with global shape modeling. 
    To this end, we propose to learn implicit surface reconstruction by sign-agnostic optimization of convolutional occupancy networks, to simultaneously achieve generality, specialty, and applicability in an integrated framework. 
    The high-level design of our approach is based on local implicit field optimization that inherits the generality of local models and the specialty of optimization strategy.  But we target sign-agnostic implicit surface optimization from un-oriented point clouds without the use of normal information, which largely improves the applicability to real scans.
    
    
    The overall pipeline of our method is illustrated in Fig.\ref{fig:pipeline}. 
    We pursue our goals through a simple yet effective strategy, a sign-agnostic optimization of occupancy field learned from convolutional features of 3D U-Net \cite{ronneberger2015u}. 
    As the occupancy decoder has already represented global signed fields after network pre-training by the accessible datasets with ground-truth signed fields, we can apply unsigned objectives that maximize the consistency between predicted occupancy fields and the inputs of un-oriented point clouds to further benefit the faithful detail generation.
    Besides, the global consistency between local fields can be naturally enforced as both local and global information is effectively aggregated in the U-Net. The property of global awareness can avoid the use of additional normal information to guide the local field assembly.
    }
    We will present more details about convolutional occupancy fields pretraining in Sec.~\ref{SecConvONet} and our proposed signed-agnostic implicit surface optimization during inference in the Sec.~\ref{SecSurfFit}.
    

==> ICCV2021 Sign Agnostic ConvONet/related.tex <==
\section{Related Work}
In this section, we briefly review existing methods for surface reconstruction from raw point clouds. Specifically, we only review those implicit reconstruction methods that find a field function (occupancy function or signed distance function) to approximate the given point cloud.
    
\noindent \textbf{Classic Optimization-based Surface Reconstruction}
% Classical methods ~\cite{alexa2003computing, carr2001reconstruction, levin2004mesh, kazhdan2006poisson, kazhdan2013screened},
 Computing a continuous surface from its discrete approximation is a severely ill-posed problem, since there could be infinitely possible solutions. Classical methods ~\cite{alexa2003computing, carr2001reconstruction, levin2004mesh, kazhdan2006poisson, kazhdan2013screened} formulate this task as a mathematical optimization problem and try to solve this problem \dan{utilizing} pre-defined geometric priors such as local linearity and smoothness. 
 There have been a number of representative reconstruction methods \dan{such as} Radius Basis Function (RBF)~\cite{carr2001reconstruction}, Moving Least Square (MLS)~\cite{alexa2003computing}, and Poisson Surface Reconstruction (PSR)~\cite{kazhdan2006poisson, kazhdan2013screened}.
 The RBF~\cite{carr2001reconstruction} represents surface as \dan{a} linear combination of a series of radial basis functions; \dan{the} MLS~\cite{alexa2003computing} fits observed points via finding those constituent spatially-varying polynomials; the PSR~\cite{kazhdan2006poisson, kazhdan2013screened} models the surface reconstruction as \dan{a} Poisson's equation.
  
 %{\color{red} classic methods are more sensitive to imperfect observations, because the modeling principles they use usually cannot deal with the noises from real scans well.}}


\noindent \textbf{Learning-based Surface Reconstruction}
More recently, driven by large-scale 3D datasets \dan{(e.g.  ShapeNet~\cite{chang2015shapenet})}, neural networks have achieved \dan{notable} successes in the field of implicit surface reconstruction from point clouds, \dan{ranging from} global to local field modeling. The global models~\cite{mescheder2019occupancy, chen2019learning} intrinsically perform shape retrieval in the latent space~\cite{tatarchenko2019single}, leading to limited generality to represent unseen shapes and restricted power to capture complex details. These drawbacks can be \dan{resolved} by the local models~\cite{chibane2020implicit, saito2019pifu, xu2019disn, peng2020convolutional, erler2020points2surf} that focus on local geometry modeling. Our method also adopts the manner of the local implicit field learning.  Thus it possesses the capability of representing large-scale scenes. Another advantage is the better generality to unseen shapes, which can provide relatively good \dan{initialization} of signed fields for the test-time optimization.

\noindent \textbf{Combination of \dan{Data-Driven} Priors and Optimization}
The above-mentioned learning methods~\cite{chibane2020implicit, saito2019pifu, xu2019disn, peng2020convolutional} fix the learned priors during inference. \dan{Specifically}, they directly obtain a 3D surface via a single feed-forward pass.
As the pre-trained priors are fixed, they have difficulty \dan{in} generalizing well to unseen shapes that are dissimilar to the training samples. 
Some existing approaches ~\cite{park2019deepsdf, jiang2020local, chabra2020deep, tretschk2020patchnets, xu2019geometry, yang2020deep, tang2021learning} try to combine the data-driven priors with optimization strategy at the test phase to acquire better results for each given input.  
Among them, the methods of local field optimization, including LIG~\cite{jiang2020local}, DeepLocalSDF~\cite{chabra2020deep}, and PatchNet~\cite{tretschk2020patchnets}, can achieve state-of-the-art performance. However, they require \emph{additional surface normals} to solve the sign flipping problem when assembling local fields into a globally consistent one, which seriously limits their applicability to raw scans that lack reliable and accurate surface normals. Our method also belongs to this line of \dan{research}. However, \dan{in contrast to} them, we optimize local implicit fields that are conditioned on the convolutional features learned in an hourglass manner. Since the global consistency between local fields can be effectively maintained in the process of hourglass convolutional feature learning, we can always guarantee the local field \dan{assemblies} as a globally consistent one during optimization, although we do not have the guidance of surface normals.

\noindent \textbf{Sign-Agnostic Surface Reconstruction}
The raw point clouds scanned by sensing devices usually lack oriented normals. Although we can approximate them via normal estimation methods~\cite{hoppe1992surface, guennebaud2007algebraic,Sheng2019Unsupervised, guerrero2018pcpnet, ben2020deepfit}, the normal estimation errors can cause degenerated surfaces. Thus it is more appealing to model surface directly from un-oriented points in a sign-agnostic manner~\cite{atzmon2020sal, atzmon2020sal++}. The SAL~\cite{atzmon2020sal} avoids the use of surface normals by properly initializing the implicit decoder network, such that they can produce signed solutions of implicit functions only using unsigned objectives. 
Our key idea of sign-agnostic implicit field optimization is similar to SAL. With the assistance of auxiliary datasets with ground-truth signed implicit fields, the occupancy decoder can be trained to represent signed fields. Given signed implicit fields as \dan{initialization} for the test-time optimization, we further adapt the pre-trained priors to the given input, by applying the unsigned cross-entropy loss to align the desired iso-surface with the observed un-oriented point cloud. 
\tang{A concurrent work of SAIL-S3~\cite{zhao2021sign} extended the geometric initialization of SAL~\cite{atzmon2020sal} for local signed field learning from un-oriented point clouds. However, it still requires a post-optimization stage to avoid the local sign flipping issue.}

%\noindent \textbf{Point Cloud Upsampling}
%%%%%
%Lastly, directly optimizing learned implicit fields towards sparse and noisy point clouds causes the phenomenon of error fitting. 

%In addition, as mentioned before, optimizing an implicit surface to be consistent with its discrete approximation of point clouds would be problematic if the observed point clouds are sparse and noisy. To this end, we use the auxiliary pre-trained model of PU-GAN~\cite{li2019pu} CAD-PU~\cite{lin2020cad} to perform patched-based point cloud upsampling~\cite{} for the inputs, which can increase the density of points and reduce the noise level. Thus we can use the denser and cleaner point clouds for unsigned objective computation. Compared to imperfect raw observation, the improved version can  provide stronger and more reliable regularization in the test-time optimization stage.
%%%%%

==> ICCV2021 Sign Agnostic ConvONet/tabs/chair.tex <==

\begin{table}[htbp]
    \vspace{-0.3cm}
        \centering
            \begin{tabular}{l|c c c c}
            \toprule
            Methods  & CD $\downarrow$ & NC $\uparrow $ & FS ($\tau$) $\uparrow$ &  FS (2$\tau$) $\uparrow$ \\ %IoU $\uparrow$ 
            \hline \hline
            SPSR \cite{kazhdan2013screened} & 1.923 & 81.54  & 80.86  & 85.13 \\     %&  52.27\\
            \hline
            ONet\cite{mescheder2019occupancy} & 1.117  & 84.58  & 62.35  & 86.57 \\  %& 55.61 \\
            SAL \cite{atzmon2020sal}          & 2.418  & 78.67  & 54.33  & 73.70 \\  % & 32.83 \\
            IGR \cite{gropp2020implicit}   & 2.678  & 75.97  & 69.02  & 76.01 \\ % & 15.37 \\
            \hline
            CONet \cite{peng2020convolutional}  & 0.821  & 91.12  & 74.73 & 96.85 \\ % & 64.03 \\
            LIG \cite{jiang2020local}      & 2.200  & 80.35   & 60.62   & 65.99 \\ % & 27.47\\
            \hline
            Ours & \textbf{0.522} & \textbf{93.51} & \textbf{97.16} & \textbf{99.37} \\  %& \textbf{70.18}  \\
            \bottomrule
            \end{tabular}
        \vspace{0.1cm}
        \caption{
        Quantitative \dan{comparison} for surface reconstruction from un-oriented point clouds on the ShapeNet-chair. }%\cite{chang2015shapenet}.}The metrics of chamfer distance (CD $\times 0.01$), normal consistency (NC $\times 0.01$), and F-score (FS $\times 0.01$) are reported.}
        \label{table:chair}
    \vspace{-0.3cm}
\end{table}


==> ICCV2021 Sign Agnostic ConvONet/tabs/method_compara.tex <==
    
    \begin{table}
        \centering
        \scalebox{0.9}{
        \begin{tabular}{l|c c c}
        \toprule
        \makecell{Methods \\} & \makecell{Without \\ normals} & \makecell{Optimization of \\ network parameters} & \makecell{Local geometry \\ modeling} \\
        % Methods & \makecell{Not require normals} & \makecell{Find optimal  results} & \makecell{Local geometry modeling} \\
        \hline \hline
        SPSR~\cite{kazhdan2013screened} & $\times$  & $\checkmark$ & $\checkmark$  \\
        \hline
        ONet~\cite{mescheder2019occupancy} & $\checkmark$ &  $\times$  & $\times$ \\
        SAL~\cite{atzmon2020sal} & $\checkmark$ & $\times$  &  $\times$ \\
        IGR~\cite{gropp2020implicit} & $\checkmark$  & $\checkmark$   & $\times$ \\
        %Point2Surf~\cite{erler2020points2surf} & $\checkmark$ & $\times$  & $\checkmark$ \\
        \hline
        %DeepSDF~\cite{park2019deepsdf} & $\times$ &   $\checkmark$  & $\times$ \\
        CONet~\cite{peng2020convolutional} & $\checkmark$ &  $\times$  & $\checkmark$ \\
        %LocalSDF~\cite{chabra2020deep} &  $\times$ &  $\checkmark$  & $\checkmark$ \\
        %PatchNets~\cite{tretschk2020patchnets} &  $\times$ &  $\checkmark$  & $\checkmark$ \\
        LIG \cite{jiang2020local} &  $\times$ &  $\checkmark$  & $\checkmark$ \\
        \hline
        Ours & $\checkmark$ & $\checkmark$  & $\checkmark$ \\
        \bottomrule
        \end{tabular}
        }
        % \vspace{-0.3cm}
        \vspace{0.1cm}
        \caption{
        \tang{Working condition summary of different methods.
        %Note that our method is the first to provide a model for learning implicit fields that can scale to large-scale scenes, generalize to unseen shapes, and be directly from real-world scans without normals, because it performs local geometry modeling, optimizes network parameters while does not use normals during inference.
        Note that our method is the first to maximize the scalability to large-scale scenes, generality to novel shapes, and applicability to real-world scans in a unified framework by performing local geometry modeling, optimizing network parameters while not requiring normals during inference.}
        }
        \label{table:compare_chara}
        \vspace{-0.3cm}
    \end{table}

==> ICCV2021 Sign Agnostic ConvONet/tabs/scannet.tex <==
\begin{table}[htbp]
    \centering
        \begin{tabular}{l|ccccc}
        \toprule
        Methods  & CD $\downarrow$ & NC $\uparrow $ & FS ($\tau$) $\uparrow$ & FS (2$\tau$) $\uparrow$  \\
        \hline\hline
        SPSR \cite{kazhdan2013screened} & 1.339 & 84.60  &  \textbf{82.33} & 87.83 \\
        \hline
        %[delete ]ONet\cite{mescheder2019occupancy}  & 7.907  & 58.52  &  11.38 / 18.98 \\
        SAL \cite{atzmon2020sal} & 2.026 & 81.24  & 61.54 & 80.90  \\
        IGR \cite{gropp2020implicit}   & 2.392 & 84.12  &  78.07  & 83.98  \\
        \hline
        CONet \cite{peng2020convolutional}  & 1.559  & 82.05  & 59.55 & 80.76 \\
        LIG \cite{jiang2020local}      & 1.501  & 81.99   & 70.39 & 78.30  \\
        \hline
        Ours & \textbf{0.728} & \textbf{86.40} & 82.08  & \textbf{95.86}\\
        \bottomrule
        \end{tabular}
    \vspace{0.1cm}
    \caption{
    Quantitative \dan{comparison} for surface reconstruction from un-oriented point clouds on the real-world ScanNet dataset \cite{peng2020convolutional}. As watertight meshes are not provided by ScanNet, we directly evaluate all methods using the pretrained models on the synthetic room dataset. } %The metrics of chamfer distance (CD $\times 0.01$), normal consistency (NC $\times 0.01$), and F-score (FS $\times 0.01$) are reported. 
    \label{table:scannet}
    \vspace{-0.3cm}
\end{table}

==> ICCV2021 Sign Agnostic ConvONet/tabs/synthetic_room.tex <==
\begin{table}[htbp]
    \vspace{-0.3cm}
    \centering
        \begin{tabular}{l|cccc}
        \toprule
        Methods  & CD $\downarrow$ & NC $\uparrow $ & FS ($\tau$) $\uparrow$ & FS (2$\tau$) $\uparrow$  \\
        \hline\hline
        SPSR \cite{kazhdan2013screened} & 2.083 & 78.21  & 76.17 & 81.22  \\
        \hline
        %[delete] ONet\cite{mescheder2019occupancy} & 14.93  & 47.75  & 4.56  /6.02 \\
        SAL \cite{atzmon2020sal}          & 2.720  & 73.85 & 40.47  &  59.79   \\
        IGR \cite{gropp2020implicit}   & 1.923 & 77.94 & 74.02 & 81.23  \\
        \hline
        CONet \cite{peng2020convolutional} & 2.020 & 83.43 & 73.28 &  81.74  \\
        LIG \cite{jiang2020local}      & 1.953 & 79.82 & 62.46 &  70.96  \\
        \hline
        Ours & \textbf{0.495} & \textbf{90.04} &  \textbf{93.85} & \textbf{98.82}   \\
        \bottomrule
        \end{tabular}
    \vspace{0.1cm}
    \caption{
    Quantitative results for surface reconstruction from un-oriented point clouds on the synthetic room dataset \cite{peng2020convolutional}.} %The metrics of chamfer distance (CD $\times 0.01$), normal consistency (NC $\times 0.01$), and F-score (FS $\times 0.01$) are reported. }
    \label{table:synthetic_room}
    \vspace{-0.3cm}
\end{table}

==> ICCV2021 Sign Agnostic ConvONet/tabs_supple/ablation.tex <==
\begin{table}[h]
    %\vspace{-0.3cm}
    \renewcommand\arraystretch{1.2}
    \setlength{\tabcolsep}{1.5mm}
        \centering
        \scalebox{0.9}{
            \begin{tabular}{l | l |c c c c}
            \toprule
            Datasets & Methods  & CD $\downarrow$ & NC $\uparrow $ & FS ($\tau$) $\uparrow$ &  FS (2$\tau$) $\uparrow$ \\ 
            \hline \hline
             \multirow{2}{*}{\shortstack{ShapaNet \\ -chair~\cite{chang2015shapenet}}}         & opt. enc. &  \textbf{0.516}  &  93.42  &   97.15 &  \textbf{99.40} \\
              & Ours & 0.522 & \textbf{93.51} & \textbf{97.16} & 99.37 \\ 
            \hline
            \multirow{2}{*}{\shortstack{Synethetic \\ Room~\cite{peng2020convolutional}}} & opt. enc. & 0.516  &  89.75  &  93.43  &  98.53 \\
                  & Ours & \textbf{0.495} & \textbf{90.04} &  \textbf{93.85} & \textbf{98.82}   \\
            \hline
            \multirow{2}{*}{ScanNet~\cite{dai2017scannet}}          & opt. enc. & 0.741  & 86.24 & 81.49 & 95.56 \\
               &Ours & \textbf{0.728} & \textbf{86.40} & \textbf{82.08}  & \textbf{95.86}\\
            % \hline
            \bottomrule
            \end{tabular}
        }
        \caption{\textbf{Additional ablation studies} on three datasets.} %The metrics of chamfer distance (CD $\times 0.01$), normal consistency (NC $\times 0.01$), and F-score (FS $\times 0.01$ with the $\tau = 0.01$) are reported.}
        \label{table:ablation}
        \vspace{-5pt}
\end{table}
%\vspace{-0.3cm}

==> ICCV2021 Sign Agnostic ConvONet/tabs_supple/ablation_sparsity.tex <==
    \begin{table}[htbp]
        %\vspace{-1pt}
        \centering
        \resizebox{0.83\linewidth}{!}{
        \begin{tabular}{l|cccc}
            \toprule
            %($\times 0.01$)  ($\%$)
             $|\mathcal{P}|$  & CD $\downarrow$ & NC $\uparrow $ & FS ($\tau$) $\uparrow$ & FS (2$\tau$) $\uparrow$  \\
            \hline\hline
            5,000   & 0.529 & 89.71 & 95.51 & 99.00   \\
            10,000  & 0.524 & 92.37 & 96.85 & 99.20   \\
            20,000  & 0.522 & 93.29 & 97.11 & 99.06   \\
            30,000  & 0.522 & 93.51 & 97.16 & 99.37   \\
            40,000  & 0.502 & 93.57 & 97.11 & 99.35   \\
            50,000  & 0.502 & 93.61 & 97.04 & 99.29   \\
            \bottomrule
        \end{tabular}
        }
        \vspace{1mm}
        \caption{ Quantitative results at different sparsity levels of
        the input point cloud $\mathcal{P}$ on the ShapeNet `chair' category.}
        \vspace{-0.2cm}
        \label{table:sparsity:chair}
    \end{table}

    \begin{table}[htbp]
        %\vspace{-1pt}
        \centering
        \resizebox{0.83\linewidth}{!}{
        \begin{tabular}{l|cccc}
            \toprule
             $|\mathcal{P}|$  & CD $\downarrow$ & NC $\uparrow $ & FS ($\tau$) $\uparrow$ & FS (2$\tau$) $\uparrow$  \\
            \hline\hline
            5,000   & 0.511 & 89.24  & 93.50 &  98.57   \\
            10,000  & 0.494 & 89.86  & 94.01 &  98.89   \\
            20,000  & 0.494 & 90.03  & 93.85 &  98.73   \\
            30,000  & 0.495 & 90.04  & 93.85 &  98.82   \\
            40,000  & 0.488 & 90.04  & 93.85 &  98.73   \\
            50,000  & 0.476 & 89.98  & 93.95 &  98.99   \\
            \bottomrule
        \end{tabular}
        }
        \caption{ Quantitative results at different sparsity levels of
        the input point cloud $\mathcal{P}$ on the synthetic room dataset.}
        %\vspace{-0.55cm}
        \label{table:sparsity:synthetic_room}
    \end{table}

==> ablation.tex <==
%\subsection{Ablation Studies}
%\noindent \textbf{Effective of Network Pretraining for Optimizing ConvONet}
%\noindent \textbf{Curvature-Adaptive point sampling for preserving fine details}

% \subsection{Robustness Evaluation} 
%     \noindent \textbf{point sets of varying noise levels.}
%     \noindent \textbf{point sets of varying sizes.}

==> problem.tex <==
%%%%V0

\section{Problem Statement}
\label{SecPro}
    Given a set of observed points $\mathcal{P} = \{\bm{p}_i \in \mathbb{R}^3 \}_{i=1}^n$, the goal of our method is to reconstruct a surface $\mathcal{S}$ that is as similar as possible to the underlying surface $\hat{\mathcal{S}}$.  The problem is pretty intractable for several reasons. On one hand, it is severely ill-posed to compute a continuous surface from its discrete approximation, since there could be infinitely possible solutions. Classic optimization-based methods try to alleviate this ambiguity by pre-defined geometric priors. Recent data-driven methods choose to learn shape priors from large-scale datasets. Nonetheless, there is still no satisfactory solution. 
    Classic methods are sensitive to imperfect observations.
    Most learning-based methods strictly fix the learned prior at the test phrase~\cite{mescheder2019occupancy}, which causes the over-smoothness of high-frequent surface details.  %Global shape optimization~\cite{park2019deepsdf, gropp2020implicit} during inference usually has limited generality to large scenes, while local surface optimization requires additional normal information to enforce the global consistency of local assembly. 
    On the other hand, the inverse problem becomes even more difficult and challenging when we consider processing real scans where reliable normals are not associated with observed points. 
    %Due to imperfection of scan acquisition, the observed points could be noisy, incomplete, and irregularly distributed. Mathematically, the given point cloud $\{\bm{p}_i\}_{i=1}^n$ could be represented as $\{\bm{x}_i+\bm{\epsilon}_i\,|\,\bm{x}_i\in \hat{\mathcal{S}}\}_{i=1}^n$, with possibly perturbations $\{\bm{\epsilon}_i\}_{i=1}^n$. The noises can increase the errors of normal estimation, which increases the uncertainty of given data and thus the difficulty of recovering clean surfaces. 
    However, exiting state-of-the-arts, which individually optimize learned local implicit field during inference, heavies rely on accurate surface normals to enforce the global consistency of local assembly. 
    Thus the normal estimation errors would increase the uncertainty of given data and the difficulty of recovering clean surfaces.
    To this end, we aim to pursue a novel approach of local implicit field optimization that inherits the advantages of local field learning and optimization strategy. But we target surface reconstruction directly from un-oriented point clouds without the use of normal information. 
    

    
\section{Approach}
\label{SecApp}
    % Karbo
    % {\color{blue}Our proposed method mainly dedicate to tackle the problem of reconstructing possibly large scenes from unoriented point clouds while recovering as many geometric details as possible presented in the observations. Since our task is to obtain a signed implicit field from an unsigned point cloud, global awareness is requisite for our network to differentiate the interior of the solid objects. To this end, we adopt a trained convolutional occupancy network as our backbone. Briefly, the network forms a feature volume via integrating per-point features in a sign-agnostic manner, then processes the volume by a 3D-UNet to aggregate both the local and global information, finally extract the surface mesh from the obtained interpolated occupancy volume via marching cubes. To ensure the reconstruction faithfully presents the input observation, we adapt the learned prior encoded in the trained network via additionally optimizing the network parameters by conforming the predictions to our observed point cloud. This can be achieved by simply minimizing the unsigned binary cross-entry loss at test phase. 
    % The overall network composition will be detailed in SectionXXX. The test-optimiztion procedure will be presented in SectionXXX.}
    
    Our proposed method is primarily motivated from the characteristic of hourglass networks such as U-Net~\cite{ronneberger2015u}, which consists of a series of down- and up-sampling convolutions with skip connections to aggregate both local and global information. 
    In this way, the final output features at different spatial positions naturally respect the global shape prior, which implicitly constraint the global consistency between local fields that are learned from these features. 
    Besides, inspired by SAL~\cite{atzmon2020sal}, we resort to auxiliary datasets with occupancy field groundtruths to pre-train our model. This can initialize the occupancy decoder as a signed field before the test-optimization. 
    Thus, different from those methods ~\cite{jiang2020local, chabra2020deep, tretschk2020patchnets} that individually optimize each local field and utilize the provided orientation information to solve the sign flipping problem between local fields, we can jointly optimize local fields by optimizing the convolutional features learned in a hourglass manner without the use of surface normals. 
    This means we do not need to consider the sign flipping problem between local fields.
    we can a self-supervised objective to maximize the consistency between learned local implicit fields and input observation.
        
     The overall pipeline of our method is illustrated in Fig.\ref{fig:pipeline}. 
     We will present more details about network architecture ( Sec.~\ref{SecUNet} and Sec.~\ref{SecOccPred}), and training paradigm (Sec.\ref{SecLoss}) to learn local shape prior and pretrain the occupancy decoder as a signed field. Next we will discuss our proposed signed-agnostic implicit surface fitting during inference in the Sec.~\ref{SecSurfFit}.
     
     
     
%%%%V1

\subsection{Overview}
\label{SubSecOver}
    Given a set of observed points $\mathcal{P} = \{\bm{p}_i \in \mathbb{R}^3 \}_{i=1}^n$, the goal of our method is to reconstruct a implicit surface $\mathcal{S}$ that is as similar as possible to the underlying surface $\hat{\mathcal{S}}$.  It is severely ill-posed to compute a continuous surface from its discrete approximation, since there could be infinitely possible solutions. Classic optimization-based methods try to alleviate this ambiguity by pre-defined geometric priors. Recent data-driven methods choose to learn shape priors from large-scale datasets to improve the robustness to imperfect observations.
    {\color{red}
    A lot of methods have been proposed  to push the progress of implicit surface reconstruction from various respects, in terms of improving generality, specialty, and applicability. But there is still not an approach that can simultaneously achieve advancements in all three respects. Most learning-based methods~\cite{mescheder2019occupancy, chen2019learning, peng2020convolutional} strictly fix the learned prior during inference, resulting in the over-smoothness of high-frequency surface details.  
    Global shape optimization~\cite{park2019deepsdf, gropp2020implicit, yang2020deep} during inference usually has limited generality to large scenes, while local surface optimization~\cite{jiang2020local, chabra2020deep, tretschk2020patchnets} requires additional normal information that are not always avaiable in real scans to enforce the global consistency of local field assembly. 
    Although SAL~\cite{atzmon2020sal} bypass the requirements of normals via sign-agnostic learning, it can only work with global shape modeling. 
    To this end, we propose to learn implicit surface reconstruction by sign-agnostic optimization of convolutional occupancy networks, to simultaneously achieve generality, specialty, and applicability in an integrated framework. 
    The high-level design of our approach is based on local implicit field optimization that inherits the generality of local models and the specialty of optimization strategy.  But we target sign-agnostic implicit surface optimization from un-oriented point clouds without the use of normal information, which largely improves the applicability to real scans.
    
    
    The overall pipeline of our method is illustrated in Fig.\ref{fig:pipeline}. 
    We pursue our goals through a simple yet effective strategy, a sign-agnostic optimization of occupancy field learned from convolutional features of 3D U-Net \cite{ronneberger2015u}. 
    As the occupancy decoder has already represented global signed fields after network pre-training by the accessible datasets with ground-truth signed fields, we can apply unsigned objectives that maximize the consistency between predicted occupancy fields and the inputs of un-oriented point clouds to further benefit the faithful detail generation.
    Besides, the global consistency between local fields can be naturally enforced as both local and global information is effectively aggregated in the U-Net. The property of global awareness can avoid the use of additional normal information to guide the local field assembly.
    }
    We will present more details about convolutional occupancy fields pretraining in Sec.~\ref{SecConvONet} and our proposed signed-agnostic implicit surface optimization during inference in the Sec.~\ref{SecSurfFit}.
    
